Pairwise Comparison Evolutionary Dynamics with Strategy-Dependent Revision Rates: Stability and Delta-Passivity (Expanded Version)

We report on new stability conditions for evolutionary dynamics in the context of population games. We adhere to the prevailing framework consisting of many agents, grouped into populations, that interact noncooperatively by selecting strategies with a favorable payoff. Each agent is repeatedly allowed to revise its strategy at a rate referred to as revision rate. Previous stability results considered either that the payoff mechanism was a memoryless potential game, or allowed for dynamics (in the payoff mechanism) at the expense of precluding any explicit dependence of the agents' revision rates on their current strategies. Allowing the dependence of revision rates on strategies is relevant because the agents' strategies at any point in time are generally unequal. To allow for strategy-dependent revision rates and payoff mechanisms that are dynamic (or memoryless games that are not potential), we focus on an evolutionary dynamics class obtained from a straightforward modification of one that stems from the so-called impartial pairwise comparison strategy revision protocol. Revision protocols consistent with the modified class retain from those in the original one the advantage that the agents operate in a fully decentralized manner and with minimal information requirements - they need to access only the payoff values (not the mechanism) of the available strategies. Our main results determine conditions under which system-theoretic passivity properties are assured, which we leverage for stability analysis.

==> RM-PC-Paper-TCNS-Version 2/bounds_Smith.tex <==

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{center}
\begin{tikzpicture}

\begin{axis}[%
width=0.5\textwidth,
height=0.5\textwidth,
scale only axis,
xmin=3,
xmax=10,
xlabel style={font=\color{white!15!black}},
xlabel={Number of strategies (n)},
xticklabel style={yshift=-4pt},
ymin=1,
ymax=10,
ylabel style={font=\color{white!15!black}},
ylabel={Bound on u/l},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
yticklabel style={xshift=-4pt},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, draw=none, mark=square, mark options={solid, mycolor1}, mark size=3pt]
table[row sep=crcr]{%
3	2\\
4	1.5\\
5	1.33333333333333\\
6	1.25\\
7	1.2\\
8	1.16666666666667\\
9	1.14285714285714\\
10	1.125\\
};
\addlegendentry{Bounds from the Corollary}

\addplot [color=mycolor2, draw=none, mark= o, mark options={solid, mycolor2}, mark size=3pt]
table[row sep=crcr]{%
3	9.44353831900066\\
4	5.89485956652755\\
5	4.65123344515052\\
6	4.00000001526338\\
7	3.59238892831641\\
8	3.30990909350444\\
9	3.1007974259754\\
10	2.93868115303495\\
};
\addlegendentry{Bounds from the Theorem}

\end{axis}
\end{tikzpicture}%
\end{center}

==> bounds_Smith.tex <==

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{center}
\begin{tikzpicture}

\begin{axis}[%
width=0.5\textwidth,
height=0.5\textwidth,
scale only axis,
xmin=3,
xmax=10,
xlabel style={font=\color{white!15!black}},
xlabel={Number of strategies (n)},
xticklabel style={yshift=-4pt},
ymin=1,
ymax=10,
ylabel style={font=\color{white!15!black}},
ylabel={Bound on u/l},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
yticklabel style={xshift=-4pt},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, draw=none, mark=square, mark options={solid, mycolor1}, mark size=3pt]
table[row sep=crcr]{%
3	2\\
4	1.5\\
5	1.33333333333333\\
6	1.25\\
7	1.2\\
8	1.16666666666667\\
9	1.14285714285714\\
10	1.125\\
};
\addlegendentry{Bounds from the Corollary}

\addplot [color=mycolor2, draw=none, mark= o, mark options={solid, mycolor2}, mark size=3pt]
table[row sep=crcr]{%
3	9.44353831900066\\
4	5.89485956652755\\
5	4.65123344515052\\
6	4.00000001526338\\
7	3.59238892831641\\
8	3.30990909350444\\
9	3.1007974259754\\
10	2.93868115303495\\
};
\addlegendentry{Bounds from the Theorem}

\end{axis}
\end{tikzpicture}%
\end{center}
